Hybrid Base Complex: Extract and Visualize Structure of Hex-dominant Meshes

Hex-dominant mesh generation has received significant attention in recent research due to its superior robustness compared to pure hex-mesh generation techniques. In this work, we introduce the first structure for analyzing hex-dominant meshes. This structure builds on the base complex of pure hex-meshes but incorporates the non-hex elements for a more comprehensive and complete representation. We provide its definition and describe its construction steps. Based on this structure, we present an extraction and categorization of sheets using advanced graph matching techniques to handle the non-hex elements. This enables us to develop an enhanced visual analysis of the structure for any hex-dominant meshes.We apply this structure-based visual analysis to compare hex-dominant meshes generated by different methods to study their advantages and disadvantages. This complements the standard quality metric based on the non-hex element percentage for hex-dominant meshes. Moreover, we propose a strategy to extract a cleaned (optimized) valence-based singularity graph wireframe to analyze the structure for both mesh and sheets. Our results demonstrate that the proposed hybrid base complex provides a coarse representation for mesh element, and the proposed valence singularity graph wireframe provides a better internal visualization of hex-dominant meshes.

==> Contents/body-sub.tex <==
\begin{document}


% \setlength{\abovedisplayskip}{-0pt}
% \setlength{\belowdisplayskip}{-0pt}
% \setlength{\abovedisplayshortskip}{3pt}
% \setlength{\belowdisplayshortskip}{2pt}
% \setlength{\belowcaptionskip}{1pt}
% \setlength{\abovecaptionskip}{2pt}
% %\setlength{\subfigtopskip}{3pt}
% \setlength{\textfloatsep}{9pt}
% \setlength{\floatsep}{3pt}
% \setlength{\intextsep}{2pt}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%% START OF THE PAPER %%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\title{Hybrid Base Complex: Extract and Visualize Structure of Hex-dominant Meshes}

\author{Lei Si, Haowei Cao, Guoning Chen~\IEEEmembership{Senior Member, IEEE}
        % <-this % stops a space
\thanks{This paper was produced by the IEEE Publication Technology Group. They are in Piscataway, NJ.}% <-this % stops a space
\thanks{Manuscript received April 19, 2021; revised August 16, 2021.}}

% The paper headers
\markboth{Journal of \LaTeX\ Class Files,~Vol.~14, No.~8, August~2021}%
{Shell \MakeLowercase{\textit{et al.}}: A Sample Article Using IEEEtran.cls for IEEE Journals}

% \IEEEpubid{0000--0000/00\$00.00~\copyright~2021 IEEE}
% Remember, if you use this you must call \IEEEpubidadjcol in t44he second
% column for its text to clear the IEEEpubid mark.

\maketitle
%-------------------------------------------------------------------------
\input{Contents/1-abstract}

\begin{IEEEkeywords}
Structure analysis, hex-dominant meshes, structure visualization
\end{IEEEkeywords}

% \input{Contents/1-teaser}
%-------------------------------------------------------------------------
\input{Contents/1-introduction}
\input{Contents/2-related-work}
\input{Contents/3-hexa-dom-base-complex}
\input{Contents/4-sheet-extraction}
\input{Contents/5-valence-based-singularity-graph}
\input{Contents/6-sheets-visualization}
\input{Contents/7-results}
\input{Contents/8-conclusion}
%-------------------------------------------------------------------------
% \clearpage


\bibliographystyle{IEEEtran}

\bibliography{Contents/paper-bibliography}

%-------------------------------------------------------------------------
\vfill
\end{document}

